Sufficient and Necessary Causal Explanations for the Analysis of Autonomous Systems

Understanding failures of autonomous systems is challenging, particularly when their behavior depends on black-box components such as neural networks. In this work, we make a distinction between two objectives of failure analysis: reproduction, which seeks to identify conditions sufficient to reproduce an observed failure, and avoidance, which seeks to identify the changes required to prevent it. Previous work on causal explanations of system failures is based on the concept of sufficient explanations and naturally supports reproduction. Nevertheless, we observe that it does not address the problem of avoiding the failure. In this paper, we introduce and formalize the concept of necessary explanations for system analysis as the correct formalism for failure avoidance. We place necessary explanations in the framework of actual causality and show that, together with sufficient explanations, they provide a unified causal framework for addressing both objectives of failure analysis. We present an efficient approximation algorithm for generating necessary explanations based on the notion of causal responsibility. We evaluate the efficiency of our approach across multiple environments. We demonstrate the practical utility of necessary explanations for failure avoidance through counterfactual generation and show that it outperforms existing methods.

==> extension.tex <==
\section{Necessary Explanation}
\label{sec:necessary}

In this section, we extend the definitions presented in \cref{subsec:cause} and introduce the notion of necessary explanations~\cite{kelly2025causal}:

\dfn[Necessary Explanation]\label{defn:necessary-exp}
A subset $\vec{V}_{nec}$ of $\vec{V}$ is a \emph{necessary explanation} of the outcome $O = 1$ if the following conditions hold:
\begin{description}
\item[{\rm EX1.}] $(M,\vec{u}_1) \models [\vec{V}_{nec} \leftarrow 0](O=0)$,
where $\vec{V}_{nec} \leftarrow 0$ stands for assigning $0$ to all variables in 
$\vec{V}_{nec}$.
\item[{\rm EX2.}] $\vec{V}_{nec}$ is minimal; there is no strict subset $\vec{V}'_{nec}$ of $\vec{V}_{nec}$ that satisfies EX1, where $\vec{v}'$ is the restriction of $\vec{v}$ to the variables in $\vec{V}'_{nec}$.
%\myv{EX1 does not refer to $\vec{V}$.}
\end{description}
\edfn

\tom{discuss the connections between the definitions }

This definition differs from \cref{defn:simple-exp} in EX1: the necessity condition starts from the original scene, $\vec{u}_1$, and focuses on a minimal subset of obstacles, such that if they were removed, the outcome would change. This is in contrast to a sufficient explanation, which starts from an empty track, $\vec{u}_0$, and looks for a minimal subset of obstacles that trigger the outcome.

The distinction between necessity and sufficiency conditions is important in environments with intricate failure-inducing factors. For example, the removal of an obstacle subset may eliminate the failure, however, this subset alone may not be sufficient to cause the crash. Less intuitively, the removal of a subset sufficient to cause the failure may not eliminate the failure, as it can be over-determined by other factors in the environment.

\tom{discuss the fact that it is the actual cause in this setting and then continue to responsibility.}

Note that the degree of responsibility in \cref{def:simple-resp} is defined with respect to a necessity condition, that is, subsets of obstacles, removing which changes the outcome. 


Necessities can be viewed as more practical in the context of CPS failure analysis. Intuitively, since failures are usually rare, finding non-failure evidence as required by EX1 in \cref{defn:necessary-exp} should be easier than finding failure evidence as required by \cref{defn:simple-exp}. \tom{Not sure it helps here}



\begin{figure}[h]
    \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[scale=0.28]{images/nec_suf_example/866.png}
        \caption{Falsifying example}
        \label{fig:orig}
    \end{subfigure}
        \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[scale=0.28]{images/nec_suf_example/2_4_5.png}
        \caption{Sufficient explanation}
        \label{fig:suf}
    \end{subfigure}
        \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[scale=0.28]{images/nec_suf_example/0_2.png}
        \caption{Necessary explanation}
        \label{fig:nec}
    \end{subfigure}
    \caption{An illustration of the difference between sufficient and necessary explanations. \cref{fig:orig} shows a falsifying example in which the vehicle crashes. \cref{fig:suf} illustrates that obstacles 3, 5, and 6 form a sufficient explanation, i.e., they alone are sufficient for the same crash as in the original scene. \cref{fig:nec} illustrates that obstacles 1 and 3 are a necessary explanation, since removing them causes the vehicle outcome to change.}
    \label{fig:nec_suf_example}
\end{figure}


\tom{link to avoidance and reproduction}

\tom{add a paragraph that discusses repair more concretely}


\tom{rewrite to link better to next section}
The precise computation of explanations is intractable~\cite{chockler2024causal}. 
%It is of little surprise, as all existing definitions in actual causality are intractable, except in some very simple special cases.
The algorithm in~\cite{icra} uses an approximate ranking---based on \emph{the degree of responsibility}---of the obstacles according to their
importance for the crash as a heuristic for the greedy construction of an explanation.
Formally, the definition of the degree of responsibility introduced in~\cite{CH04} quantifies
the definition of an \emph{actual cause}. We first introduce the definition of an actual
cause and then the definition of responsibility. For conciseness,
we introduce simplified definitions that apply to 
depth-$2$ causal models (although not necessarily binary) as we use in this
paper. The reader is referred to~\cite{Hal15,Hal19} for the general definitions.

\dfn[Actual Cause \cite{HP01b}]\label{def:AC}
A subset $\vec{V}_{ac} \subseteq \vec{V}$ and its values $\vec{v}_{ac}$ is an 
\emph{actual cause} of the outcome $O=o$ in
$(M,\vec{u})$ if the following conditions hold:
\begin{description}
\item[{\rm AC1.}] $(M,\vec{u}) \models (\vec{V}_{ac} = \vec{v}_{ac})\wedge(O=o)$. In other words,
in the context $\vec{u}$, indeed $\vec{V}_{ac} = \vec{v}_{ac}$ and $O=o$.
\item[{\rm AC2.}] There exists an assignment $\vec{v}'_{ac}$ such that 
$(M,\vec{u}) \models [\vec{V}_{ac} \leftarrow \vec{v}'_{ac}](O\not=o)$. That is, changing the values of
$\vec{V}_{ac}$ to $\vec{v}'_{ac}$ changes the outcome, if
all other variables remain unchanged.
\item[{\rm AC3.}] $\vec{V}_{ac}$ is minimal; there is no strict subset $\vec{V}'$ of $\vec{V}_{ac}$ that satisfies AC2.
\end{description}
A variable $v$ that is a part of an actual cause $\vec{V}_{ac}$ is a \emph{part of a cause}.
Following~\cite{Hal15}, we often refer to parts of causes as causes.
\edfn

\dfn[Responsibility \cite{CH04}]\label{def:simple-resp}
The \emph{degree of responsibility} of $v_i$ for the outcome $O=o$ is defined as
$1/|\vec{V}_{n}|$, where $\vec{V}_{n} \subseteq \vec{V}$ is a smallest actual cause for $O=o$ that 
contains $v_i$. 
%That is, removing any obstacle in $\vec{V}_{n}$ changes the outcome, and $\vec{V}_{n}$ is minimal.
If there is no actual cause containing $v_i$, its degree of responsibility is defined as $0$.
\edfn






==> intro_old.tex <==
\section{Introduction}

% autonmous systems fail
Autonomous Systems, whether Cyber-Physical Systems (CPSs), such as autonomous vehicles, or virtual ones, like Artificial Intelligence (AI) chat agents, are becoming an integral part of modern life~\cite{cps} \KE{wrong ref?}. These systems are expected to demonstrate ``intelligent'' behaviour, while operating in real-world, unrestricted conditions. To achieve this, the complexity of modern system design most often grows to a point where its formal analysis and end-to-end verification become intractable. This issue is further amplified by the fact that these systems often also rely on external, ``black-box'' components, such as Neural controllers, perception modules, and language interfaces (LLMs)~\cite{varshney2019deepcontrol,wang2021bounding} \KE{check these refs}. These conditions, in turn, mean that modern systems are typically only tuned empirically, making the encounter with system failures inevitable.

% failure explanation is important
Motivated by the growing interest in eXplainable Artificial Intelligence (XAI)~\cite{hoenig2024explainable,moosavi2024explainable}, this paper is concerned with the objective of failure analysis, and, more specifically, post-hoc failure explanation for black-box systems; meaning, given a specific, observed failure scenario of a system with an unknown design, after it occurred, explain it. An explanation should help us gain insight into what affected the system behaviour, which led to the failure outcome. Addressing this goal requires answering two questions: first, what counts as an explanation? Second, how to generate the right one? 

The ability to properly explain system failures is a crucial part of the system life-cycle. Prior to deployment, in the design stage, seeking, observing, and explaining failures (or ``bugs'') is integral to the design-improvement process. Post-deployment, explanation of unfortunate failures is crucial to improving safety, by guiding the user in providing guardrails, to ensure similar failures do not repeat, or make sure appropriate mitigation measures are in place in the future; in some case, it may even potentially be used online, to allow for immediate intervention and repair, in order to make sure the current task can still be achieved.

% if it is a cps, we assume we can simulate the system

% the gap: other methods for failure explantion, and why they are not enough [small part of the contribution]
To position this work clearly, we should first mention the underlying conceptual contribution of this paper (which we discuss in detail in \cref{sec:concept}, with which we identify the two complementary explanation objectives: \emph{outcome avoidance}, and \emph{outcome reproduction}. In the first case, our concern is \emph{changing} the outcome (with minimal effort), e.g., when we wish to repair the failure; the explanation should hence provide insight on which elements in the scenario should be changed (and how), in order to change the (failing) outcome.
In the second case, our concern is generating additional scenarios, in which the same (failing) outcome is \emph{maintained}, e.g., as part of a debugging process; the explanation should hence provide insight on which elements in the scenario are sufficient to recreate the outcome, regardless of the rest. The two forms of explanation are complementary, but one cannot be deduced from the other.

These two objectives also logically correspond to the two main categories in the existing body of work on failure explanation.
Works in the first category (e.g.,~\cite{ghazal2026towards,han2025counterfactual,manca2023explainable}) address the objective of outcome avoidance by providing mechanisms for counterfactual generation, i.e., generation of ``similar'' scenarios (to the given failure example), in which the outcome is different (no longer failing). 
Works in the second category (e.g.,~\cite{narteni2022sensitivity,diwakaran2017}) address the objective of outcome reproduction through sensitivity analysis, i.e., identifying regions of the scenario-input values (around the nominal example), for which the (failure) outcome is preserved.
Yet, both of these approaches, to their respective objectives, only provide an implicit, superficial form of explanation.


% exaplaining failures with actual causailty and core contribution
Diverging from these two approaches, a recent promising work~\cite{icra} suggested using the framework of ``actual causality''~\cite{Hal16,CH24} to formally define and generate \emph{causal} failure explanations (for CPSs). That work provided a rigorous yet practical point of view, building on prior work, where the framework had been used to explain decisions of image and audio classifiers~\cite{CKKS26,kelly_i_2026,yaacov2026causal}. While providing a step in the right direction, we also recognize that that work's scope was limited. According to our categorization, that work only addressed the objective of failure reproduction, by focusing on the generation of ``sufficient explanations'' (an established concept in actual causality, which they applied to failure explanation). Such explanation are qualitatively not suitable to serve the objective of failure avoidance.
This work seeks to extend the foundations laid in~\cite{icra}, to also address the objective of failure avoidance, by applying the concept of ``necessary explanations'' from the framework of actual causality. Together, this would provide, for the first time, a unified (causal) formal framework for failure analysis, allowing to address both objectives. As exact computation of such causal explanations may quickly become intractable, when the number of inputs increases~\cite{CKKS26}, we also developed a practical, scalable algorithm, capable of generating approximate explanations according to the computation budget. 
Proving that this form of explanation provides a deeper-level insight, once a necessary explanation is found, one can naturally generate a counterfactual example from it as a downstream artifact, by modifying the inputs accordingly, and re-running the system.

We summarize our contributions: 
(i) We suggest a conceptual categorization to the objectives of failure explanation---a critical step in understanding, comparing, and advancing contributions in this field. (ii) We qualitatively extend the causal failure-explanation framework established in \cite{icra}, with the concept of \emph{necessary explanations}, allowing to use the framework to address the explanation objective of \emph{failure avoidance}. (iii) We develop a practical, scalable explanation generation algorithm and provide an experimental evaluation of its efficiency (compared to brute-force computation), demonstrating its quantitative benefit. Finally, to prove the superiority of this this framework for explanation for failure avoidance, (iv) we provide a a study comparing the counterfactuals generated using common baselines, and those generated as an artifact of our causal explanations; we show that our approach achieves higher success rate, lower computation time, and better quality (more similar to the source) counterfactuals.
For clarity, the paper is presented (and contributions (iii) and (iv) are evaluated) using a running example of an autonomous car with a black-box neural controller, trained to avoid collisions (as in \cref{fig:car}). In our evaluation, we use two autonomous driving simulators, of both high and low fidelity, showing the benefits of our approach are simulator and system independent.


\KE{The paper is structured} as follows: \cref{sec:prelim} provides preliminaries on the system testing-model, and introduces the running example. \cref{sec:ac-for-cps} presents the fundamental framework of actual causality for failure explanation. \cref{sec:concept} includes a discussion on our conceptual contribution, introducing a novel taxonomy for explanation objectives. \cref{sec:ac-for-cps} presents our theoretical contribution, extending the said framework with necessary explanations, to support the objective of failure avoidance. \cref{sec:algorithm} presents the practical algorithm for computing necessary explanations, with its experimental efficiency evaluation in \cref{sec:performance-evaluation}. \cref{sec:counterfactuals-evaluation} demonstrates the usage and utility of necessary explanations for failure avoidance through counterfactual generation. \cref{sec:conclusion} concludes the paper.


\begin{comment}
Autonomous systems rely on algorithms and digital computation to control real-world machines and achieve complex objectives autonomously~\cite{cps} \KE{wrong ref?}. As these objectives become increasingly challenging, modern systems have come to rely heavily on black-box components, such as neural networks~\cite{varshney2019deepcontrol,wang2021bounding}. The opacity of these components, combined with the complexity of systems and the variability of their operating environments, makes it difficult to interpret system behavior and gain insight into how decisions were made.
This difficulty has motivated the rapidly growing interest in Explainable Artificial Intelligence (XAI), which is widely regarded as crucial for the widespread adoption of autonomous systems~\cite{hoenig2024explainable,moosavi2024explainable}. 
% XAI comprises a broad family of techniques designed to provide insight into the behavior of deep learning models, thereby improving understanding of and trust in their predictions. Post-hoc XAI is one type of XAI, where explanations are generated for individual instances after the model has been trained.

Explainability becomes even more vital when failures happen. Understanding failures, known as \emph{failure analysis}, is crucial for the development and debugging of systems, and it is especially challenging when systems rely on black-box components, often provided by a third party. 
Post-hoc XAI, where explanations are generated for individual instances after the model has been trained, are
a suitable paradigm for analyzing black-box components, as it does not require any changes or even access to 
the internals of the component, and it is the one we follow in this paper.

% \hrule


% \KE{The point here should (only) be: the type of (failure) explanation in use nowadays are ``sufficient'' (like in our previous paper...) But here we recognize that, esp. in the context of failure explanation, this type of explanation might not always be useful/desirable, as it is not repair-oriented. Hence, we identify the need for a different, more appropriate type of explanation.}

\textbf{Problem definition:} Given a failing execution, the analysis goal is to be able to \textbf{reproduce} it, generate \textbf{additional similar failing executions}, and
to introduce minimal changes to \textbf{avoid} or repair the failure. 

In this work, we make the distinction between two objectives above that failure explanations can serve: \emph{reproduction} and \emph{avoidance}. Failure reproduction aims to identify and understand the conditions responsible for a failure and to leverage this understanding for tasks such as reproducing the current failure and generating additional failure cases for more thorough correctness analysis. Failure avoidance seeks to determine which elements of a failing scenario should be modified so that the failure is avoided. This can be viewed as the first step towards failure repair. 

The most relevant existing approach to failure reproduction is based on the application of \emph{actual causality} 
to isolate the sufficient causes for failure~\cite{icra}. 
%Existing explainability approaches for failure reproduction include sensitivity analysis~\cite{narteni2022sensitivity,diwakaran2017} and, more recently, the application of \emph{actual causality} to isolate the sufficient causes for failure~\cite{icra}. 
A set of sufficient causes (a sufficiency) is a subset of the elements of the failure execution that is, by itself, sufficient to result in a failure. Beyond making it easier to understand why the failure occurred, it can be used to generate more failures that are based on the same sufficiency and, consequently, result in the same type of failure. This, however, does not address the second objective---avoidance.

%These methods, however, 
%do not address the second objective---avoidance. 
Crucially, we observe that an \textbf{explanation suitable for failure reproduction is not necessarily suitable for failure avoidance}, since one cannot be derived from the other: a set of conditions responsible for a failure does not naturally correspond to a set of elements whose modification eliminates the failure. We discuss this distinction in more detail in~\Cref{sec:ac-for-cps}. Thus, reproduction and avoidance pose different explanation questions and require different causal notions. Failure avoidance requires identifying how a given failing scenario can be modified so that the failure no longer occurs. 

 
% \tom{Find additional downsides of current work on counterfactuals}

% \hrule
We formalize an explainability approach for failure avoidance that is based on the rigorous theory of actual causality. Previous work used actual causality to introduce \emph{sufficient explanations} as a way to isolate the causes of failure and generate multiple similar failure scenarios~\cite{icra}. In this paper, we introduce the concept of \emph{necessary explanations}, which are subsets of elements of a failure scenario whose modification eliminates the failure. A minimal necessary explanation is, essentially, a minimal repair of the failing scenario that is guaranteed to remove the failure. As the exact computation is intractable in all but very small cases~\cite{CKKS26}, we introduce an approximation algorithm for computing these explanations and evaluate it. 
We further compare our approach with existing failure-avoidance methods based on searching for counterfactuals---passing scenarios similar to the original failing scenario. We show that our method is more efficient and finds smaller repair candidates.
% We evaluate this algorithm and compare it to existing approaches, such as counterfactual-based ones, demonstrating that our algorithm is more efficient and finds smaller candidates for repair. 

\textbf{Our approach puts the reproduction and the avoidance objectives in a single formal framework of actual causality and allows to tackle them using the same toolkit of methods that actual causality supports}. Actual causality provides a high degree of flexibility with respect to the problem setup. 
For instance, it allows us to distinguish between repairable and unrepairable (fixed) elements of the scenario by defining different types of variables. It also supports different levels of granularity, for example, by manipulating obstacles (removal vs. changing position) or other elements of the scenario. It also allows us to incorporate prior expert knowledge in the form of structural equations, defining how elements interact and their inter-dependencies, or allowed ranges of variables. This eliminates unrealistic or infeasible repair suggestions. \textbf{In this work, we treat the autonomous
system's controller as a black box}, but incorporating knowledge about its inner workings, if exists and needed, is possible. \KE{?}
\tom{elaborate more about this black box discussion}

% The problem is thus to leverage the framework of actual causality for failure analysis. Specifically, we aim to


\textbf{Conributions:} The paper contributions are: \textbf{(1)} We \textbf{introduce the notion of necessary explanations for autonomous system failures} and discuss its application to system failure analysis. \textbf{(2)} We \textbf{distinguish between failure reproduction and avoidance
and provide a unified causal framework for analyzing both, based on sufficient and necessary explanations}, respectively. We discuss the distinction between these two notions and illustrate how they support different objectives of failure analysis. \textbf{(3)} We present an \textbf{efficient algorithm for generating necessary explanations}, guided by the quantitative notion of causal responsibility~\cite{CH04,Hal19}. We empirically evaluate the algorithm across multiple environments and demonstrate its effectiveness and efficiency. \textbf{(4)} We \textbf{demonstrate the practical utility of necessary explanations for failure avoidance} through counterfactual generation. Our empirical evaluation shows that using necessary explanations to guide the counterfactual search produces more targeted counterfactuals and outperforms existing methods.
%\KE{Needs to sharpen the contribution structure. Should be clear that the paper has two/three essentially independent sections (novel theoretical idea, efficient algorithm, using it to generate counterfactual)}

The paper is structured as follows: \cref{sec:prelim} provides preliminaries on the autonomous system testing model, actual causality, and introduces the running example. \cref{sec:ac-for-cps} presents our theoretical contribution, introducing actual causality for system failures and extending the framework with necessary explanations, formalizing failure reproduction and avoidance through sufficient and necessary explanations, respectively. \cref{sec:algorithm} presents the approximation algorithm for computing necessary explanations. The experimental evaluation is presented in \cref{sec:performance-evaluation}. \cref{sec:counterfactuals-evaluation} demonstrates the practical utility of necessary explanations for failure avoidance through counterfactual generation. \cref{sec:conclusion} concludes the paper.


\noindent\textbf{Related Work:} 
Actual causality~\cite{Hal16,CH24} provides a formal framework for explaining specific observed outcomes. In explainable AI, causal explanations have been used in various domains, such as images~\cite{CKKS26}, audio~\cite{kelly_i_2026}, and process mining~\cite{yaacov2026causal}. 
%Since computing actual causes is generally hard, these approaches approximate causal responsibility to efficiently find causal explanations~\cite{CKK25}. These approaches, like ours, treat the AI model as a black box.

In the context of autonomous systems, failure reproduction methods seek conditions that are sufficient to recreate an observed failure. Sensitivity analysis is a type of failure reproduction that examines neighborhoods around falsifying traces, identifying regions where a property is violated~\cite{narteni2022sensitivity,diwakaran2017}. Actual causality has also been proposed for failure, providing a more structured, high-level alternative by identifying minimal subsets of environmental elements that reproduce the observed failure~\cite{icra}.


Failure avoidance methods focus on modifications to a failing scenario that change its outcome. Existing approaches primarily use counterfactual generation to produce a similar passing example~\cite{ghazal2026towards,han2025counterfactual,manca2023explainable}. 
While counterfactuals can provide valuable insight into the observed behavior, they focus on input-output changes rather than the underlying causal mechanisms, potentially attributing importance to downstream effects and including modifications that are not necessary for avoiding the failure. 
% While counterfactuals can provide valuable insight into the observed behavior, they focus on input-output changes and, consequently, may obscure the underlying causal mechanisms. Moreover, since these explanations are provided as examples, a user may attribute responsibility for failure to variables whose values change as downstream consequences of the true cause, rather than identifying the actual causal factors responsible for the failure. Consequently, a counterfactual may contain modifications that are not necessary for avoiding the failure, providing a larger and less targeted repair than required.
Autonomous systems work on explainability also uses counterfactual attribution for root-cause analysis~\cite{fang2026counterfactual}, which relies on causal discovery, 
%Such methods address important debugging and explanation questions, 
%but rely on causal discovery, 
a fundamentally different approach from actual causality.
\end{comment}

==> notes_from_meetings <==
ANALYSIS OF OF FAILURES OF CPS \KE{(Potential magazine article)}

Liveness (task completion) vs. safety\\
Planner vs. control\\
Failing within planning vs. in execution\\
Sufficient vs. necessary\\
Repair at the same iteration vs. repair the system for future iterations\\
Failure in real world vs. in simulation (catastrophic or not, sim2real "upside down", gaps between model and the world)\\
Cost of interventions (in the physical world vs in the simulation)


==> prelim_old.tex <==

Connecting the two previous formalisms, we wish to build a causal model for a test of the autonomous system, to allow for its formal analysis.
It is important to note a model is built specifically for each test, and not to the system in general.

Since we are dealing with a black-box system, we may only build a simple, depth-2 causal model $M_s$ as follows:
The set $\V = \vec{V} \cup \{O\}$ of model variables consists of a set $\vec{V}$ of Boolean variables, corresponding to the elements in $\env$, and a single binary outcome variable $O$. 
Essentially, $\vec{V}$ is a Boolean \emph{mask} indicating which elements are maintained and which are ``removed,'' to allow us to perform basic interventions on $\env$. The outcome variable $O$ indicates whether the outcome of the simulation (status) of this masked scene matches that of the original scene. That is, 
\begin{equation}
    O \doteq [\status(\statetraj,\env)\?\status(\statetraj',\env')],
\end{equation}
where $\env'$ is the environment induced by the (possibly intervened) causal setting, and $\statetraj'$ is its resulting trajectory. 
The first layer (of structural equations) in the model captures the masking and the entire simulation, connecting the element mask $\vec{V}$ to the simulation output (status). The second layer connect the status to $O$, capturing the outcome comparison.
This model is system agnostic. Having access to knowledge on the system or environment models may allow us to construct a more complex causal model, to support a richer analysis---though this is beyond the scope of this work.

==> runs_plot.tex <==
% ------------------------------------------------------------------
% Plot styles
% ------------------------------------------------------------------
\pgfplotsset{
    exhaustiveNecessary/.style={
        color=red!80,
        very thick,
        mark=*,
        mark size=1.3pt
    },
    discrete50Necessary/.style={
        color=blue!50,
        thick,
        mark=square*,
        mark size=1.3pt
    },
    discrete100Necessary/.style={
        color=blue!100,
        thick,
        mark=triangle*,
        mark size=1.5pt
    }
}

% ------------------------------------------------------------------
% Plot all three methods from one CSV
% ------------------------------------------------------------------
\newcommand{\plotnecessary}[1]{%
    \addplot[exhaustiveNecessary]
        table[
            x=obstacles,
            y=exhaustive,
            col sep=comma
        ] {#1};

    \addplot[discrete50Necessary]
        table[
            x=obstacles,
            y=discrete_25,
            col sep=comma
        ] {#1};

    \addplot[discrete100Necessary]
        table[
            x=obstacles,
            y=discrete_50,
            col sep=comma
        ] {#1};
}

% ------------------------------------------------------------------
% Same, but also creates the common legend
% ------------------------------------------------------------------
\newcommand{\plotnecessarywithlegend}[1]{%
    \addplot[exhaustiveNecessary]
        table[
            x=obstacles,
            y=exhaustive,
            col sep=comma
        ] {#1};
    \addlegendentry{Exhaustive}

    \addplot[discrete50Necessary]
        table[
            x=obstacles,
            y=discrete_25,
            col sep=comma
        ] {#1};
    \addlegendentry{Discrete 25}

    \addplot[discrete100Necessary]
        table[
            x=obstacles,
            y=discrete_50,
            col sep=comma
        ] {#1};
    \addlegendentry{Discrete 50}
}


\begin{figure*}[t]
    \centering

    \begin{tikzpicture}

        \begin{groupplot}[
            group style={
                group name=necessaryplots,
                group size=4 by 1,
                horizontal sep=8mm
            },
            width=0.28\textwidth,
            height=0.22\textwidth,
            xmin=14.7,
            xmax=19.3,
            xtick={15,16,17,18,19},
            scaled y ticks=false,
            tick align=outside,
            tick pos=left,
            grid=major,
            grid style={black!10},
            axis line style={black!60},
            tick label style={
                font=\scriptsize
            },
            label style={
                font=\small
            },
            title style={
                font=\small
            }
        ]

        % ============================================================
        % Short Narrow
        % ============================================================

        \nextgroupplot[
            title={Short Narrow},
            xlabel={Obstacles},
            ylabel={Runs},
            legend columns=3,
            legend to name=necessarylegend,
            legend style={
                font=\small,
                draw=none,
                /tikz/every even column/.append style={
                    column sep=5mm
                }
            }
        ]
        \plotnecessarywithlegend{results/sinusoidal_short_narrow_necessary_explanations_runs_results.csv}


        % ============================================================
        % Short Wide
        % ============================================================

        \nextgroupplot[
            title={Short Wide},
            xlabel={Obstacles}
        ]
        \plotnecessary{results/segmented_short_wide_necessary_explanations_runs_results.csv}


        % ============================================================
        % Long Narrow
        % ============================================================

        \nextgroupplot[
            title={Long Narrow},
            xlabel={Obstacles}
        ]
        \plotnecessary{results/lane_shift_long_narrow_necessary_explanations_runs_results.csv}


        % ============================================================
        % Long Wide
        % ============================================================

        \nextgroupplot[
            title={Long Wide},
            xlabel={Obstacles}
        ]
        \plotnecessary{results/metadrive_mixed_necessary_explanations_runs_results.csv}

        \end{groupplot}


        % ============================================================
        % COMMON LEGEND
        % ============================================================

        \node[
            anchor=north
        ] at ([yshift=-11mm]
             $(necessaryplots c1r1.south)!0.5!(necessaryplots c4r1.south)$)
        {\pgfplotslegendfromname{necessarylegend}};

    \end{tikzpicture}

    \caption{%
        Number of runs required for finding necessary explanations
        in the sinusoidal environments.
    }
    \label{fig:necessary-explanations-runs}

\end{figure*}


